A Fluorescent Material Model for Non-Spectral Editing & Rendering

Fluorescent materials are characterized by a spectral reradiation toward longer wavelengths. Recent work [Fichet et al. 2024] has shown that the rendering of fluorescence in a non-spectral engine is possible through the use of appropriate reduced reradiation matrices. But the approach has limited expressivity, as it requires the storage of one reduced matrix per fluorescent material, and only works with measured fluorescent assets. In this work, we introduce an analytical approach to the editing and rendering of fluorescence in a non-spectral engine. It is based on a decomposition of the reduced reradiation matrix, and an analytically-integrable Gaussian-based model of the fluorescent component. The model reproduces the appearance of fluorescent materials accurately, especially with the addition of a UV basis. Most importantly, it grants variations of fluorescent material parameters in real-time, either for the editing of fluorescent materials, or for the dynamic spatial variation of fluorescence properties across object surfaces. A simplified one-Gaussian fluorescence model even allows for the artist-friendly creation of plausible fluorescent materials from scratch, requiring only a few reflectance colors as input.

==> Figures/DE/content_red_cmp_xyzu.tex <==

\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/y dir=plus,
        /pgfplots/error bars/y explicit,
        /pgfplots/table/x index=\pgfkeysvalueof{/pgfplots/box plot x index},
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot box top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
        },
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker top index}}
        },
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker bottom index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker bottom index}}
        },
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot,
        /pgfplots/table/y index=\pgfkeysvalueof{/pgfplots/box plot median index}
    },
    box plot width/.initial=1em,
    box plot x index/.initial=0,
    box plot median index/.initial=1,
    box plot box top index/.initial=2,
    box plot box bottom index/.initial=3,
    box plot whisker top index/.initial=4,
    box plot whisker bottom index/.initial=5,
}

\newcommand{\boxplot}[2][]{
    \addplot [box plot median,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot box,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot top whisker,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot bottom whisker,#1] table[col sep=comma] {#2};
}

\begin{tikzpicture}
    \begin{axis} [
        name=moustache,
        box plot width=1.2mm,
        enlargelimits=false,
        width=\linewidth,
        height=4cm,
        xmin=0.25,
        xmax=8.75,
        xtick=data,
        xtick={1,...,8},
        xticklabels from table={Figures/DE/data/illu.csv}{Illuminant},
        x tick label style={rotate=45,anchor=east,font=\tiny},
        y tick label style={font=\tiny},
        ylabel={\tiny{$\Delta E_{2000}^*$}},
        ylabel near ticks,
        ]
        \boxplot [
            thick,
            blue,
            fill=blue!30!white,
            forget plot,
            box plot whisker bottom index=2,
            box plot box bottom index=3,
            box plot median index=1,
            box plot box top index=5,
            box plot whisker top index=6
        ] {Figures/DE/data/with_diag/de_patches_1-tabulated_fit-xyzu.csv}

        \boxplot [
            thick,
            red,
            fill=red!30!white,
            forget plot,
            box plot whisker bottom index=2,
            box plot box bottom index=3,
            box plot median index=1,
            box plot box top index=5,
            box plot whisker top index=6
        ] {Figures/DE/data/with_diag/de_patches_1-analytic-xyzu.csv}
    \end{axis}

    \node[xshift=.5cm, yshift=-0.15cm, anchor=north west] (key_g1) at (moustache.north west) {\scriptsize{Tabulated reduction on fit}};
    \node[xshift=.5cm, yshift=-0.45cm, anchor=north west] (key_g2) at (moustache.north west) {\scriptsize{Analytical reduction}};

    \draw[blue,fill=blue!30!white]            ($(key_g1.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g1.west) - (.1cm, 0) - (.1cm, .1cm)$);
    \draw[red,fill=red!30!white]              ($(key_g2.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g2.west) - (.1cm, 0) - (.1cm, .1cm)$);
\end{tikzpicture}

==> Figures/DE/reduction_xyz.tex <==
\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/y dir=plus,
        /pgfplots/error bars/y explicit,
        /pgfplots/table/x index=\pgfkeysvalueof{/pgfplots/box plot x index},
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot box top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
        },
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker top index}}
        },
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker bottom index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker bottom index}}
        },
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot,
        /pgfplots/table/y index=\pgfkeysvalueof{/pgfplots/box plot median index}
    },
    box plot width/.initial=1em,
    box plot x index/.initial=0,
    box plot median index/.initial=1,
    box plot box top index/.initial=2,
    box plot box bottom index/.initial=3,
    box plot whisker top index/.initial=4,
    box plot whisker bottom index/.initial=5,
}

\newcommand{\boxplot}[2][]{
    \addplot [box plot median,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot box,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot top whisker,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot bottom whisker,#1] table[col sep=comma] {#2};
}


\begin{tikzpicture}
    \begin{axis} [
        name=moustache,
        box plot width=0.8mm,
        enlargelimits=false,
        width=\linewidth,
        height=4cm,
        xmin=0.25,
        xmax=8.75,
        xtick=data,
        xtick={1,...,8},
        xticklabels from table={Figures/DE/data/illu.csv}{Illuminant},
        x tick label style={rotate=45,anchor=east,font=\tiny},
        y tick label style={font=\tiny},
        ylabel={\tiny{$\Delta E_{2000}^*$}},
        ylabel near ticks,
        ]
        \boxplot [
            thick,
            blue,
            fill=blue!30!white,
            forget plot,
            box plot whisker bottom index=2,
            box plot box bottom index=3,
            box plot median index=1,
            box plot box top index=5,
            box plot whisker top index=6
        ] {Figures/DE/data/reduction_xyz/tbl_DE_R_reduction_diag.csv}

        %\boxplot [
        %    thick,
        %    red,
        %    fill=red!30!white,
        %    forget plot,
        %    box plot whisker bottom index=2,
        %    box plot box bottom index=3,
        %    box plot median index=1,
        %    box plot box top index=5,
        %    box plot whisker top index=6
        %] {data/reduction_xyz/tbl_DE_R_reduction_ref.csv}

        \boxplot [
            thick,
            brown,
            fill=brown!30!white,
            forget plot,
            box plot whisker bottom index=2,
            box plot box bottom index=3,
            box plot median index=1,
            box plot box top index=5,
            box plot whisker top index=6
        ] {Figures/DE/data/reduction_xyz/tbl_DE_R_reduction_Rxyz.csv}
    \end{axis}

    \node[xshift=-1.5cm, yshift=-0.15cm, anchor=north west] (key_g1) at (moustache.north east) {\scriptsize{diagonal}};
    %\node[xshift=-2.5cm, yshift=-0.55cm, anchor=north west] (key_g2) at (moustache.north east) {\scriptsize{Numerical reduction}};
    \node[xshift=-1.5cm, yshift=-0.45cm, anchor=north west] (key_g3) at (moustache.north east) {\scriptsize{upscaling}};

    \draw[blue,fill=blue!30!white]            ($(key_g1.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g1.west) - (.1cm, 0) - (.1cm, .1cm)$);
    %\draw[red,fill=red!30!white]              ($(key_g2.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g2.west) - (.1cm, 0) - (.1cm, .1cm)$);
    \draw[brown!60!black,fill=brown!30!white] ($(key_g3.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g3.west) - (.1cm, 0) - (.1cm, .1cm)$);
\end{tikzpicture}



==> Figures/DE/reduction_xyz_chroma.tex <==
\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/y dir=plus,
        /pgfplots/error bars/y explicit,
        /pgfplots/table/x index=\pgfkeysvalueof{/pgfplots/box plot x index},
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot box top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
        },
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker top index}}
        },
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker bottom index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker bottom index}}
        },
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot,
        /pgfplots/table/y index=\pgfkeysvalueof{/pgfplots/box plot median index}
    },
    box plot width/.initial=1em,
    box plot x index/.initial=0,
    box plot median index/.initial=1,
    box plot box top index/.initial=2,
    box plot box bottom index/.initial=3,
    box plot whisker top index/.initial=4,
    box plot whisker bottom index/.initial=5,
}

\newcommand{\boxplot}[2][]{
    \addplot [box plot median,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot box,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot top whisker,#1] table[col sep=comma] {#2};
    \addplot [forget plot, box plot bottom whisker,#1] table[col sep=comma] {#2};
}


\begin{tikzpicture}
    \begin{axis} [
        name=moustache,
        box plot width=0.8mm,
        enlargelimits=false,
        width=\linewidth,
        height=4cm,
        xmin=0.25,
        xmax=8.75,
        xtick=data,
        xtick={1,...,8},
        xticklabels from table={Figures/DE/data/illu.csv}{Illuminant},
        x tick label style={rotate=45,anchor=east,font=\tiny},
        y tick label style={font=\tiny},
        ylabel={\tiny{RMSE}},
        ylabel near ticks,
        ]
        \boxplot [
            thick,
            blue,
            fill=blue!30!white,
            forget plot,
            box plot whisker bottom index=2,
            box plot box bottom index=3,
            box plot median index=1,
            box plot box top index=5,
            box plot whisker top index=6
        ] {Figures/DE/data/reduction_xyz/tbl_rmse_R_reduction_diag.csv}

        %\boxplot [
        %    thick,
        %    red,
        %    fill=red!30!white,
        %    forget plot,
        %    box plot whisker bottom index=2,
        %    box plot box bottom index=3,
        %    box plot median index=1,
        %    box plot box top index=5,
        %    box plot whisker top index=6
        %] {data/reduction_xyz/tbl_DE_R_reduction_ref.csv}

        \boxplot [
            thick,
            brown,
            fill=brown!30!white,
            forget plot,
            box plot whisker bottom index=2,
            box plot box bottom index=3,
            box plot median index=1,
            box plot box top index=5,
            box plot whisker top index=6
        ] {Figures/DE/data/reduction_xyz/tbl_rmse_R_reduction_Rxyz.csv}
    \end{axis}

    \node[xshift=-1.5cm, yshift=-0.15cm, anchor=north west] (key_g1) at (moustache.north east) {\scriptsize{diagonal}};
    %\node[xshift=-2.5cm, yshift=-0.55cm, anchor=north west] (key_g2) at (moustache.north east) {\scriptsize{Numerical reduction}};
    \node[xshift=-1.5cm, yshift=-0.45cm, anchor=north west] (key_g3) at (moustache.north east) {\scriptsize{upscaling}};

    \draw[blue,fill=blue!30!white]            ($(key_g1.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g1.west) - (.1cm, 0) - (.1cm, .1cm)$);
    %\draw[red,fill=red!30!white]              ($(key_g2.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g2.west) - (.1cm, 0) - (.1cm, .1cm)$);
    \draw[brown!60!black,fill=brown!30!white] ($(key_g3.west) - (.1cm, 0) + (.1cm, .1cm)$) rectangle ($(key_g3.west) - (.1cm, 0) - (.1cm, .1cm)$);
\end{tikzpicture}



==> Figures/PalettesMatrix/figure.tex <==
\begin{figure}
    % \center
    \resizebox{\linewidth}{!}{
    \input{./Figures/PalettesMatrix/figure_weak.tex}
    }
    \vspace{-15pt}
    \caption{
	\textbf{Influence of albedo and emission location on the fluorescence.}
    }
    \label{fig:palette_matrix}
\end{figure}


==> Figures/PalettesMatrix/figure_moderate.tex <==
\begin{figure}[h!]
\begin{tikzpicture}[font=\footnotesize]
% \newlength{\x}
\setlength{\x}{0.19\linewidth}
\begin{scope}
	% First line
	\node[inner sep=0pt] (Moderate_red0)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/0-render-red.jpg} };
	\draw[black] (Moderate_red0.south west) rectangle (Moderate_red0.north east);
	\node[inner sep=0pt, right=2pt of Moderate_red0] (Moderate_yellow0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/0-render-yellow.jpg} };
	\draw[black] (Moderate_yellow0.south west) rectangle (Moderate_yellow0.north east);
	\node[inner sep=0pt, right=2pt of Moderate_yellow0] (Moderate_green0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/0-render-green.jpg} };
	\draw[black] (Moderate_green0.south west) rectangle (Moderate_green0.north east);       	
	\node[inner sep=0pt, right=2pt of Moderate_green0] (Moderate_blue0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/0-render-blue.jpg} };
	\draw[black] (Moderate_blue0.south west) rectangle (Moderate_blue0.north east);    	
	\node[inner sep=0pt, right=2pt of Moderate_blue0] (Moderate_pink0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/0-render-pink.jpg} };
	\draw[black] (Moderate_pink0.south west) rectangle (Moderate_pink0.north east);
		\draw[black, thin]  (Moderate_red0.north) -- (Moderate_red0.south);
		\draw[black, thin]  (Moderate_yellow0.north) -- (Moderate_yellow0.south);
		\draw[black, thin]  (Moderate_green0.north) -- (Moderate_green0.south);
		\draw[black, thin]  (Moderate_blue0.north) -- (Moderate_blue0.south);
		\draw[black, thin]  (Moderate_pink0.north) -- (Moderate_pink0.south);
		\node[color=white, anchor=south west, above=0pt of Moderate_red0.south west,xshift= 0.25\x] {$D65$};
		\node[color=white, anchor=south east, above=0pt of Moderate_red0.south east,xshift=-0.25\x] {$UV$};

	% Second line
	\node[inner sep=0pt, below=2pt of Moderate_red0] (Moderate_red1)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/1-render-red.jpg} };
	\draw[black] (Moderate_red1.south west) rectangle (Moderate_red1.north east);
	\node[inner sep=0pt, right=2pt of Moderate_red1] (Moderate_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/1-render-yellow.jpg} };
	\draw[black] (Moderate_yellow.south west) rectangle (Moderate_yellow.north east);
	\node[inner sep=0pt, right=2pt of Moderate_yellow] (Moderate_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/1-render-green.jpg} };
	\draw[black] (Moderate_green.south west) rectangle (Moderate_green.north east);       	
	\node[inner sep=0pt, right=2pt of Moderate_green] (Moderate_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/1-render-blue.jpg} };
	\draw[black] (Moderate_blue.south west) rectangle (Moderate_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Moderate_blue] (Moderate_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/1-render-pink.jpg} };
	\draw[black] (Moderate_pink.south west) rectangle (Moderate_pink.north east);
		\draw[black, thin]  (Moderate_red1.north) -- (Moderate_red1.south);
		\draw[black, thin]  (Moderate_yellow.north) -- (Moderate_yellow.south);
		\draw[black, thin]  (Moderate_green.north) -- (Moderate_green.south);
		\draw[black, thin]  (Moderate_blue.north) -- (Moderate_blue.south);
		\draw[black, thin]  (Moderate_pink.north) -- (Moderate_pink.south);
	
	% Third line
	\node[inner sep=0pt, below=2pt of Moderate_red1] (Moderate_red2)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/2-render-red.jpg} };
	\draw[black] (Moderate_red2.south west) rectangle (Moderate_red2.north east);
	\node[inner sep=0pt, right=2pt of Moderate_red2] (Moderate_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/2-render-yellow.jpg} };
	\draw[black] (Moderate_yellow.south west) rectangle (Moderate_yellow.north east);
	\node[inner sep=0pt, right=2pt of Moderate_yellow] (Moderate_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/2-render-green.jpg} };
	\draw[black] (Moderate_green.south west) rectangle (Moderate_green.north east);       	
	\node[inner sep=0pt, right=2pt of Moderate_green] (Moderate_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/2-render-blue.jpg} };
	\draw[black] (Moderate_blue.south west) rectangle (Moderate_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Moderate_blue] (Moderate_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/2-render-pink.jpg} };
	\draw[black] (Moderate_pink.south west) rectangle (Moderate_pink.north east);
		\draw[black, thin]  (Moderate_red2.north) -- (Moderate_red2.south);
		\draw[black, thin]  (Moderate_yellow.north) -- (Moderate_yellow.south);
		\draw[black, thin]  (Moderate_green.north) -- (Moderate_green.south);
		\draw[black, thin]  (Moderate_blue.north) -- (Moderate_blue.south);
		\draw[black, thin]  (Moderate_pink.north) -- (Moderate_pink.south);

	% Fourth line
	\node[inner sep=0pt, below=2pt of Moderate_red2] (Moderate_red3)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/3-render-red.jpg} };
	\draw[black] (Moderate_red3.south west) rectangle (Moderate_red3.north east);
	\node[inner sep=0pt, right=2pt of Moderate_red3] (Moderate_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/3-render-yellow.jpg} };
	\draw[black] (Moderate_yellow.south west) rectangle (Moderate_yellow.north east);
	\node[inner sep=0pt, right=2pt of Moderate_yellow] (Moderate_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/3-render-green.jpg} };
	\draw[black] (Moderate_green.south west) rectangle (Moderate_green.north east);       	
	\node[inner sep=0pt, right=2pt of Moderate_green] (Moderate_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/3-render-blue.jpg} };
	\draw[black] (Moderate_blue.south west) rectangle (Moderate_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Moderate_blue] (Moderate_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/3-render-pink.jpg} };
	\draw[black] (Moderate_pink.south west) rectangle (Moderate_pink.north east);
		\draw[black, thin]  (Moderate_red3.north) -- (Moderate_red3.south);
		\draw[black, thin]  (Moderate_yellow.north) -- (Moderate_yellow.south);
		\draw[black, thin]  (Moderate_green.north) -- (Moderate_green.south);
		\draw[black, thin]  (Moderate_blue.north) -- (Moderate_blue.south);
		\draw[black, thin]  (Moderate_pink.north) -- (Moderate_pink.south);

	% Fifth line
	\node[inner sep=0pt, below=2pt of Moderate_red3] (Moderate_red4)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/4-render-red.jpg} };
	\draw[black] (Moderate_red4.south west) rectangle (Moderate_red4.north east);
	\node[inner sep=0pt, right=2pt of Moderate_red4] (Moderate_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/4-render-yellow.jpg} };
	\draw[black] (Moderate_yellow.south west) rectangle (Moderate_yellow.north east);
	\node[inner sep=0pt, right=2pt of Moderate_yellow] (Moderate_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/4-render-green.jpg} };
	\draw[black] (Moderate_green.south west) rectangle (Moderate_green.north east);       	
	\node[inner sep=0pt, right=2pt of Moderate_green] (Moderate_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/4-render-blue.jpg} };
	\draw[black] (Moderate_blue.south west) rectangle (Moderate_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Moderate_blue] (Moderate_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Moderate/4-render-pink.jpg} };
	\draw[black] (Moderate_pink.south west) rectangle (Moderate_pink.north east);
		\draw[black, thin]  (Moderate_red4.north) -- (Moderate_red4.south);
		\draw[black, thin]  (Moderate_yellow.north) -- (Moderate_yellow.south);
		\draw[black, thin]  (Moderate_green.north) -- (Moderate_green.south);
		\draw[black, thin]  (Moderate_blue.north) -- (Moderate_blue.south);
		\draw[black, thin]  (Moderate_pink.north) -- (Moderate_pink.south);

		% Title on columns
		\node[inner sep=0pt, above=2pt of Moderate_red0]   { $h =   0$ };
		\node[inner sep=0pt, above=2pt of Moderate_yellow0]{ $h = 0.16$ };
		\node[inner sep=0pt, above=2pt of Moderate_green0] { $h = 0.38$ };
		\node[inner sep=0pt, above=2pt of Moderate_blue0]  { $h = 0.64$ };
		\node[inner sep=0pt, above=2pt of Moderate_pink0]  { $h = 0.83$ };

		% Title on lines
		\node[inner sep=0pt, rotate=90, left=2pt of Moderate_red0, anchor=south] { $ \mu_e = 451 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Moderate_red1, anchor=south] { $ \mu_e = 505 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Moderate_red2, anchor=south] { $ \mu_e = 539 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Moderate_red3, anchor=south] { $ \mu_e = 573 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Moderate_red4, anchor=south] { $ \mu_e = 588 $ };
\end{scope}
    \end{tikzpicture}
\caption{\textbf{Appearance matrix with moderate fluorescence strength}. Fluorescence already predominates in the final color.
\label{fig:moderate-matrix}
}
\end{figure}

==> Figures/PalettesMatrix/figure_strong.tex <==
\begin{figure}[h!]
\begin{tikzpicture}[font=\footnotesize]
% \newlength{\x}
\setlength{\x}{0.19\linewidth}
\begin{scope}
	% First line
	\node[inner sep=0pt] (Strong_red0)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/0-render_red.jpg} };
	\draw[black] (Strong_red0.south west) rectangle (Strong_red0.north east);
	\node[inner sep=0pt, right=2pt of Strong_red0] (Strong_yellow0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/0-render_yellow.jpg} };
	\draw[black] (Strong_yellow0.south west) rectangle (Strong_yellow0.north east);
	\node[inner sep=0pt, right=2pt of Strong_yellow0] (Strong_green0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/0-render_green.jpg} };
	\draw[black] (Strong_green0.south west) rectangle (Strong_green0.north east);       	
	\node[inner sep=0pt, right=2pt of Strong_green0] (Strong_blue0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/0-render_blue.jpg} };
	\draw[black] (Strong_blue0.south west) rectangle (Strong_blue0.north east);    	
	\node[inner sep=0pt, right=2pt of Strong_blue0] (Strong_pink0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/0-render_pink.jpg} };
	\draw[black] (Strong_pink0.south west) rectangle (Strong_pink0.north east);
		\draw[black, thin]  (Strong_red0.north) -- (Strong_red0.south);
		\draw[black, thin]  (Strong_yellow0.north) -- (Strong_yellow0.south);
		\draw[black, thin]  (Strong_green0.north) -- (Strong_green0.south);
		\draw[black, thin]  (Strong_blue0.north) -- (Strong_blue0.south);
		\draw[black, thin]  (Strong_pink0.north) -- (Strong_pink0.south);
		\node[color=white, anchor=south west, above=0pt of Strong_red0.south west,xshift= 0.25\x] {$D65$};
		\node[color=white, anchor=south east, above=0pt of Strong_red0.south east,xshift=-0.25\x] {$UV$};

	% Second line
	\node[inner sep=0pt, below=2pt of Strong_red0] (Strong_red1)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/1-render_red.jpg} };
	\draw[black] (Strong_red1.south west) rectangle (Strong_red1.north east);
	\node[inner sep=0pt, right=2pt of Strong_red1] (Strong_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/1-render_yellow.jpg} };
	\draw[black] (Strong_yellow.south west) rectangle (Strong_yellow.north east);
	\node[inner sep=0pt, right=2pt of Strong_yellow] (Strong_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/1-render_green.jpg} };
	\draw[black] (Strong_green.south west) rectangle (Strong_green.north east);       	
	\node[inner sep=0pt, right=2pt of Strong_green] (Strong_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/1-render_blue.jpg} };
	\draw[black] (Strong_blue.south west) rectangle (Strong_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Strong_blue] (Strong_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/1-render_pink.jpg} };
	\draw[black] (Strong_pink.south west) rectangle (Strong_pink.north east);
		\draw[black, thin]  (Strong_red1.north) -- (Strong_red1.south);
		\draw[black, thin]  (Strong_yellow.north) -- (Strong_yellow.south);
		\draw[black, thin]  (Strong_green.north) -- (Strong_green.south);
		\draw[black, thin]  (Strong_blue.north) -- (Strong_blue.south);
		\draw[black, thin]  (Strong_pink.north) -- (Strong_pink.south);
	
	% Third line
	\node[inner sep=0pt, below=2pt of Strong_red1] (Strong_red2)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/2-render_red.jpg} };
	\draw[black] (Strong_red2.south west) rectangle (Strong_red2.north east);
	\node[inner sep=0pt, right=2pt of Strong_red2] (Strong_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/2-render_yellow.jpg} };
	\draw[black] (Strong_yellow.south west) rectangle (Strong_yellow.north east);
	\node[inner sep=0pt, right=2pt of Strong_yellow] (Strong_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/2-render_green.jpg} };
	\draw[black] (Strong_green.south west) rectangle (Strong_green.north east);       	
	\node[inner sep=0pt, right=2pt of Strong_green] (Strong_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/2-render_blue.jpg} };
	\draw[black] (Strong_blue.south west) rectangle (Strong_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Strong_blue] (Strong_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/2-render_pink.jpg} };
	\draw[black] (Strong_pink.south west) rectangle (Strong_pink.north east);
		\draw[black, thin]  (Strong_red2.north) -- (Strong_red2.south);
		\draw[black, thin]  (Strong_yellow.north) -- (Strong_yellow.south);
		\draw[black, thin]  (Strong_green.north) -- (Strong_green.south);
		\draw[black, thin]  (Strong_blue.north) -- (Strong_blue.south);
		\draw[black, thin]  (Strong_pink.north) -- (Strong_pink.south);

	% Fourth line
	\node[inner sep=0pt, below=2pt of Strong_red2] (Strong_red3)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/3-render_red.jpg} };
	\draw[black] (Strong_red3.south west) rectangle (Strong_red3.north east);
	\node[inner sep=0pt, right=2pt of Strong_red3] (Strong_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/3-render_yellow.jpg} };
	\draw[black] (Strong_yellow.south west) rectangle (Strong_yellow.north east);
	\node[inner sep=0pt, right=2pt of Strong_yellow] (Strong_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/3-render_green.jpg} };
	\draw[black] (Strong_green.south west) rectangle (Strong_green.north east);       	
	\node[inner sep=0pt, right=2pt of Strong_green] (Strong_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/3-render_blue.jpg} };
	\draw[black] (Strong_blue.south west) rectangle (Strong_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Strong_blue] (Strong_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/3-render_pink.jpg} };
	\draw[black] (Strong_pink.south west) rectangle (Strong_pink.north east);
		\draw[black, thin]  (Strong_red3.north) -- (Strong_red3.south);
		\draw[black, thin]  (Strong_yellow.north) -- (Strong_yellow.south);
		\draw[black, thin]  (Strong_green.north) -- (Strong_green.south);
		\draw[black, thin]  (Strong_blue.north) -- (Strong_blue.south);
		\draw[black, thin]  (Strong_pink.north) -- (Strong_pink.south);

	% Fifth line
	\node[inner sep=0pt, below=2pt of Strong_red3] (Strong_red4)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/4-render_red.jpg} };
	\draw[black] (Strong_red4.south west) rectangle (Strong_red4.north east);
	\node[inner sep=0pt, right=2pt of Strong_red4] (Strong_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/4-render_yellow.jpg} };
	\draw[black] (Strong_yellow.south west) rectangle (Strong_yellow.north east);
	\node[inner sep=0pt, right=2pt of Strong_yellow] (Strong_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/4-render_green.jpg} };
	\draw[black] (Strong_green.south west) rectangle (Strong_green.north east);       	
	\node[inner sep=0pt, right=2pt of Strong_green] (Strong_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/4-render_blue.jpg} };
	\draw[black] (Strong_blue.south west) rectangle (Strong_blue.north east);    	
	\node[inner sep=0pt, right=2pt of Strong_blue] (Strong_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Strong/4-render_pink.jpg} };
	\draw[black] (Strong_pink.south west) rectangle (Strong_pink.north east);
		\draw[black, thin]  (Strong_red4.north) -- (Strong_red4.south);
		\draw[black, thin]  (Strong_yellow.north) -- (Strong_yellow.south);
		\draw[black, thin]  (Strong_green.north) -- (Strong_green.south);
		\draw[black, thin]  (Strong_blue.north) -- (Strong_blue.south);
		\draw[black, thin]  (Strong_pink.north) -- (Strong_pink.south);

		% Title on columns
		\node[inner sep=0pt, above=2pt of Strong_red0]   { $h =   0$ };
		\node[inner sep=0pt, above=2pt of Strong_yellow0]{ $h = 0.16$ };
		\node[inner sep=0pt, above=2pt of Strong_green0] { $h = 0.38$ };
		\node[inner sep=0pt, above=2pt of Strong_blue0]  { $h = 0.64$ };
		\node[inner sep=0pt, above=2pt of Strong_pink0]  { $h = 0.83$ };

		% Title on lines
		\node[inner sep=0pt, rotate=90, left=2pt of Strong_red0, anchor=south] { $ \mu_e = 451 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Strong_red1, anchor=south] { $ \mu_e = 505 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Strong_red2, anchor=south] { $ \mu_e = 539 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Strong_red3, anchor=south] { $ \mu_e = 573 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of Strong_red4, anchor=south] { $ \mu_e = 588 $ };
\end{scope}
    \end{tikzpicture}
\caption{\textbf{Appearance matrix with strong fluorescence strength}. Fluorescence clearly predominates in the final color.
\label{fig:strong-matrix}
}
\end{figure}

==> Figures/PalettesMatrix/figure_weak.tex <==
\begin{figure}[h!]
\begin{tikzpicture}[font=\footnotesize]
% \newlength{\x}
\setlength{\x}{0.19\linewidth}
\begin{scope}
	% First line
	\node[inner sep=0pt] (weak_red0)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/0-render-red.jpg} };
	\draw[black] (weak_red0.south west) rectangle (weak_red0.north east);
	\node[inner sep=0pt, right=2pt of weak_red0] (weak_yellow0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/0-render-yellow.jpg} };
	\draw[black] (weak_yellow0.south west) rectangle (weak_yellow0.north east);
	\node[inner sep=0pt, right=2pt of weak_yellow0] (weak_green0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/0-render-green.jpg} };
	\draw[black] (weak_green0.south west) rectangle (weak_green0.north east);       	
	\node[inner sep=0pt, right=2pt of weak_green0] (weak_blue0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/0-render-blue.jpg} };
	\draw[black] (weak_blue0.south west) rectangle (weak_blue0.north east);    	
	\node[inner sep=0pt, right=2pt of weak_blue0] (weak_pink0) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/0-render-pink.jpg} };
	\draw[black] (weak_pink0.south west) rectangle (weak_pink0.north east);
		\draw[black, thin]  (weak_red0.north) -- (weak_red0.south);
		\draw[black, thin]  (weak_yellow0.north) -- (weak_yellow0.south);
		\draw[black, thin]  (weak_green0.north) -- (weak_green0.south);
		\draw[black, thin]  (weak_blue0.north) -- (weak_blue0.south);
		\draw[black, thin]  (weak_pink0.north) -- (weak_pink0.south);
		\node[color=white, anchor=south west, above=0pt of weak_red0.south west,xshift= 0.25\x] {$D65$};
		\node[color=white, anchor=south east, above=0pt of weak_red0.south east,xshift=-0.25\x] {$UV$};

	% Second line
	\node[inner sep=0pt, below=2pt of weak_red0] (weak_red1)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/1-render-red.jpg} };
	\draw[black] (weak_red1.south west) rectangle (weak_red1.north east);
	\node[inner sep=0pt, right=2pt of weak_red1] (weak_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/1-render-yellow.jpg} };
	\draw[black] (weak_yellow.south west) rectangle (weak_yellow.north east);
	\node[inner sep=0pt, right=2pt of weak_yellow] (weak_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/1-render-green.jpg} };
	\draw[black] (weak_green.south west) rectangle (weak_green.north east);       	
	\node[inner sep=0pt, right=2pt of weak_green] (weak_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/1-render-blue.jpg} };
	\draw[black] (weak_blue.south west) rectangle (weak_blue.north east);    	
	\node[inner sep=0pt, right=2pt of weak_blue] (weak_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/1-render-pink.jpg} };
	\draw[black] (weak_pink.south west) rectangle (weak_pink.north east);
		\draw[black, thin]  (weak_red1.north) -- (weak_red1.south);
		\draw[black, thin]  (weak_yellow.north) -- (weak_yellow.south);
		\draw[black, thin]  (weak_green.north) -- (weak_green.south);
		\draw[black, thin]  (weak_blue.north) -- (weak_blue.south);
		\draw[black, thin]  (weak_pink.north) -- (weak_pink.south);
	
	% Third line
	\node[inner sep=0pt, below=2pt of weak_red1] (weak_red2)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/2-render-red.jpg} };
	\draw[black] (weak_red2.south west) rectangle (weak_red2.north east);
	\node[inner sep=0pt, right=2pt of weak_red2] (weak_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/2-render-yellow.jpg} };
	\draw[black] (weak_yellow.south west) rectangle (weak_yellow.north east);
	\node[inner sep=0pt, right=2pt of weak_yellow] (weak_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/2-render-green.jpg} };
	\draw[black] (weak_green.south west) rectangle (weak_green.north east);       	
	\node[inner sep=0pt, right=2pt of weak_green] (weak_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/2-render-blue.jpg} };
	\draw[black] (weak_blue.south west) rectangle (weak_blue.north east);    	
	\node[inner sep=0pt, right=2pt of weak_blue] (weak_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/2-render-pink.jpg} };
	\draw[black] (weak_pink.south west) rectangle (weak_pink.north east);
		\draw[black, thin]  (weak_red2.north) -- (weak_red2.south);
		\draw[black, thin]  (weak_yellow.north) -- (weak_yellow.south);
		\draw[black, thin]  (weak_green.north) -- (weak_green.south);
		\draw[black, thin]  (weak_blue.north) -- (weak_blue.south);
		\draw[black, thin]  (weak_pink.north) -- (weak_pink.south);

	% Fourth line
	\node[inner sep=0pt, below=2pt of weak_red2] (weak_red3)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/3-render-red.jpg} };
	\draw[black] (weak_red3.south west) rectangle (weak_red3.north east);
	\node[inner sep=0pt, right=2pt of weak_red3] (weak_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/3-render-yellow.jpg} };
	\draw[black] (weak_yellow.south west) rectangle (weak_yellow.north east);
	\node[inner sep=0pt, right=2pt of weak_yellow] (weak_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/3-render-green.jpg} };
	\draw[black] (weak_green.south west) rectangle (weak_green.north east);       	
	\node[inner sep=0pt, right=2pt of weak_green] (weak_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/3-render-blue.jpg} };
	\draw[black] (weak_blue.south west) rectangle (weak_blue.north east);    	
	\node[inner sep=0pt, right=2pt of weak_blue] (weak_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/3-render-pink.jpg} };
	\draw[black] (weak_pink.south west) rectangle (weak_pink.north east);
		\draw[black, thin]  (weak_red3.north) -- (weak_red3.south);
		\draw[black, thin]  (weak_yellow.north) -- (weak_yellow.south);
		\draw[black, thin]  (weak_green.north) -- (weak_green.south);
		\draw[black, thin]  (weak_blue.north) -- (weak_blue.south);
		\draw[black, thin]  (weak_pink.north) -- (weak_pink.south);

	% Fifth line
	\node[inner sep=0pt, below=2pt of weak_red3] (weak_red4)    { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/4-render-red.jpg} };
	\draw[black] (weak_red4.south west) rectangle (weak_red4.north east);
	\node[inner sep=0pt, right=2pt of weak_red4] (weak_yellow) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/4-render-yellow.jpg} };
	\draw[black] (weak_yellow.south west) rectangle (weak_yellow.north east);
	\node[inner sep=0pt, right=2pt of weak_yellow] (weak_green) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/4-render-green.jpg} };
	\draw[black] (weak_green.south west) rectangle (weak_green.north east);       	
	\node[inner sep=0pt, right=2pt of weak_green] (weak_blue) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/4-render-blue.jpg} };
	\draw[black] (weak_blue.south west) rectangle (weak_blue.north east);    	
	\node[inner sep=0pt, right=2pt of weak_blue] (weak_pink) { \includegraphics[width=\x]{./Figures/PalettesMatrix/Weak/4-render-pink.jpg} };
	\draw[black] (weak_pink.south west) rectangle (weak_pink.north east);
		\draw[black, thin]  (weak_red4.north) -- (weak_red4.south);
		\draw[black, thin]  (weak_yellow.north) -- (weak_yellow.south);
		\draw[black, thin]  (weak_green.north) -- (weak_green.south);
		\draw[black, thin]  (weak_blue.north) -- (weak_blue.south);
		\draw[black, thin]  (weak_pink.north) -- (weak_pink.south);

		% Title on columns
		\node[inner sep=0pt, above=2pt of weak_red0]   { $h =   0$ };
		\node[inner sep=0pt, above=2pt of weak_yellow0]{ $h = 0.16$ };
		\node[inner sep=0pt, above=2pt of weak_green0] { $h = 0.38$ };
		\node[inner sep=0pt, above=2pt of weak_blue0]  { $h = 0.64$ };
		\node[inner sep=0pt, above=2pt of weak_pink0]  { $h = 0.83$ };

		% Title on lines
		\node[inner sep=0pt, rotate=90, left=2pt of weak_red0, anchor=south] { $ \mu_e = 451 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of weak_red1, anchor=south] { $ \mu_e = 505 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of weak_red2, anchor=south] { $ \mu_e = 539 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of weak_red3, anchor=south] { $ \mu_e = 573 $ };
		\node[inner sep=0pt, rotate=90, left=2pt of weak_red4, anchor=south] { $ \mu_e = 588 $ };
\end{scope}
\end{tikzpicture}
\caption{\textbf{Appearance matrix with weak fluorescence strength}. Fluorescence and reflectance are combined in the final color.
\label{fig:weak-matrix}
}
\end{figure}
